Approximating Nash Equilibria in Tree Polymatrix Games

We develop a quasi-polynomial time Las Vegas algorithm for approximating Nash equilibria in polymatrix games over trees, under a mild renormalizing assumption. Our result, in particular, leads to an expected polynomial-time algorithm for computing approximate Nash equilibria of tree polymatrix games in which the number of actions per player is a fixed constant. Further, for trees with constant degree, the running time of the algorithm matches the best known upper bound for approximating Nash equilibria in bimatrix games (Lipton, Markakis, and Mehta 2003). Notably, this work closely complements the hardness result of Rubinstein (2015), which establishes the inapproximability of Nash equilibria in polymatrix games over constant-degree bipartite graphs with two actions per player.

==> related-work.tex <==
Computing Approximate Nash Equilibria in Polymatrix Games -- Computation of $0.5 + \delta$-Nash equilibrium 

Inapproximability of Nash equilibrium -- Rubinstein 
We complement this hardness result. It shows that there exists a constant $\delta$ such that finding an $\delta$-Nash equilibrium in polymatrix games over bipartite graphs of constant degree is computationally hard. Our complementary result pushes against this work. 

Polymatrix games are central in the PPAD-hardness results for Nash and approximate Nash equilibria. E.g., the reductions developed in Daskalakis, Goldberg, and Papadimitriou along with Chen, Deng, and Teng critically employ polymatrix games. 


Nash equilibria in graphical games on trees revisited---this work studies equilibrium computation in graphical games (with two actions per player) on bounded-degree trees. Our framework subsumes this prior work. 


Zero-Sum Polymatrix games:
1. On minmax theorems for multiplayer games 
2. On a network generalization of the minmax theorem




Old references that study polymatrix games:
1. Yanovskaya E B (1968) Equilibrium points in polymatrix games, (in Russian) Lithuanian Mathematical Journal

2. Equilibria of polymatrix games - Howson (1972)


